Leveraging Cognitive Features for Sentiment Analysis

Sentiments expressed in user-generated short text and sentences are nuanced by subtleties at lexical, syntactic, semantic and pragmatic levels. To address this, we propose to augment traditional features used for sentiment analysis and sarcasm detection, with cognitive features derived from the eye-movement patterns of readers. Statistical classification using our enhanced feature set improves the performance (F-score) of polarity detection by a maximum of 3.7% and 9.3% on two datasets, over the systems that use only traditional features. We perform feature significance analysis, and experiment on a held-out dataset, showing that cognitive features indeed empower sentiment analyzers to handle complex constructs.

==> featureTable.tex <==
%\keepXColumns
%\begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash\hsize=0.4\hsize}X|>{\raggedright\arraybackslash\hsize=1.0\hsize}X|>{\raggedright\arraybackslash\hsize=0.25\hsize}X|>{\raggedright\arraybackslash\hsize=2.05\hsize}X|}
\begin{table*}[t]
\centering
%\scriptsize
\begin{tabular}{p{5cm}|p{11cm}}
\hline
\hline
\textbf{Feature Name} & \textbf{Intent} \\
\hline
\multicolumn{2}{c}{{\bf Category: Sentiment Features (Source: Liu and Zhang, 2012)}} \\
\hline
Unigrams (NGRAM_PCA) & Presence of unigrams in the training corpus \\
\hline
Subjective words & Presence of positive, negative and subjective words (using MPQA lexicon)\\
\hline
Subjective scores (PosScore, NegScore) & Scores of positive subjectivity and negative subjectivity using SentiWordNet \\
\hline
Sentiment flip count (EXP) & Number of times sentiment flips in the text \\
\hline
PoS ratios (VERB, NOUN, ADJ, ADV) & Ratios (proportions) of verbs, nouns, adjectives and adverbs in the text. \\
\hline
Named entity (NE) & Number of named entity mentions in the text \\
\hline
Discourse connectors (DC) & Number of discourse connectors in the text \\
\hline
\multicolumn{2}{c}{{\bf Category: Sarcasm Features (Source: Ramteke et al.,2013; Riloff et al., 2013; Joshi et al., 2015)}} \\
\hline
Implicit incongruity (IMPLICIT_PCA) & Presence of Positive phrases followed by negative situational phrase (computed using bootstrapping technique suggested by Riloff et al.) \\
\hline
Punctuation marks (PUNC) & Count of punctuation marks in the text \\
\hline
Largest pos/neg subsequence (LAR) & Length of the largest series of words with polarities unchanged \\
\hline
Lexical polarity (LP) & Sentence polarity found by supervised logistic regression \\
\hline
\multicolumn{2}{c}{{\bf Category: Cognitive Features - Textual. We introduce these features in the current work.}} \\
\hline
Readability (RED) & Flesch Readability Ease score of the sentence \\
\hline
Length (LEN) & Number of words in the sentence \\
\hline
\multicolumn{2}{c}{{\bf Category: Cognitive Features - Basic Gaze Attributes. We introduce these features in the current work.}} \\
\hline
Avg. Fixation Duration (FDUR) & Sum of fixation duration divided by word count \\
\hline
Avg. Fixation Count (FC) & Sum of fixation counts divided by word count \\
\hline
Avg. Saccade Length (SL) & Sum of saccade lengths (measured by number of words) divided by word count \\
\hline
Regression Count (REG) & Total number of gaze regressions \\
\hline
Skip count (SKIP) & Number of words skipped divided by total word count \\
\hline
Count of regressions from second half to first half of the sentence (RSF) & Number of regressions from second half of the sentence to the first half of the sentence (given the sentence is divided into two equal half of words) \\
\hline
Largest Regression Position (LREG) & Ratio of the absolute position of the word from which a regression with the largest amplitude (number of pixels) is observed, to the total word count of sentence \\
\hline
\multicolumn{2}{c}{{\bf Category: Cognitive Features - Complex Gaze Attributes. We introduce these features in the current work.}} \\
\hline
Edge density of the saliency gaze graph (ED) & Ratio of the number of directed edges to vertices in the saliency gaze graph (SGG) \\
\hline
Fixation Duration at Left/Source (F1H, F1S) & Largest weighted degree (LWD) and second largest weighted degree (SWD) of the SGG considering the fixation duration of word $i$ of edge $E_{ij}$ \\
\hline
Fixation Duration at Right/Target (F2H, F2S) & LWD and SWD of the SGG considering the fixation duration of word $j$ of edge $E_{ij}$ \\
\hline
Forward Saccade Word Count of Source (PSH, PSS) & LWD and SWD of the SGG considering the number of forward saccades between words $i$ and $j$ of an edge $E_{ij}$ \\
\hline
Forward Saccade Word Count of Destination (PSDH, PSDS) & LWD and SWD of the SGG considering the total distance (word count) of forward saccades between words $i$ and $j$ of an edge $E_{ij}$ \\
\hline
Regressive Saccade Word Count of Source (RSH, RSS) & LWD and SWD of the SGG considering the number of regressive saccades between words $i$ and $j$ of an edge $E_{ij}$ \\
\hline
Regressive Saccade Word Count of Destination (RSDH, RSDS) & LWD and SWD of the SGG considering the total distance (word count) of regressive saccades between words $i$ and $j$ of an edge $E_{ij}$ \\
\hline
\hline
\end{tabular}
%\end{tabularx}
\vspace{-0.05in}
\caption{The complete set of features used in our system.}
\label{tab:featureset}
\vspace{-0.15in}
\end{table*}

